XAI meets LLMs: A Survey of the Relation between Explainable AI and Large Language Models

In this survey, we address the key challenges in Large Language Models (LLM) research, focusing on the importance of interpretability. Driven by increasing interest from AI and business sectors, we highlight the need for transparency in LLMs. We examine the dual paths in current LLM research and eXplainable Artificial Intelligence (XAI): enhancing performance through XAI and the emerging focus on model interpretability. Our paper advocates for a balanced approach that values interpretability equally with functional advancements. Recognizing the rapid development in LLM research, our survey includes both peer-reviewed and preprint (arXiv) papers, offering a comprehensive overview of XAI's role in LLM research. We conclude by urging the research community to advance both LLM and XAI fields together.

==> benchmark_table.tex <==


\begin{table*}[ht]

\scriptsize
% \tiny
\centering
\resizebox{2\columnwidth}{!}{%
\begin{tabular}{
>{\hspace{0pt}}m{0.29\linewidth}
>{\hspace{0pt}}m{0.04\linewidth}
>{\hspace{0pt}}m{0.04\linewidth}
>{\hspace{0pt}}m{0.08\linewidth}
>{\hspace{0pt}}m{0.2\linewidth}
>{\hspace{0pt}}m{0.11\linewidth}
>{\hspace{0pt}}c} 
\toprule
\textbf{Paper and Tool} & \textbf{Star} & \textbf{Fork} & \textbf{Update} & \textbf{Target} & \textbf{Agnostic} & \textbf{Goal} \\ 
\midrule
\cite{vig2019multiscale} \href{https://github.com/jessevig/bertviz}{BertViz} & 6.1k & 734 & 08/23 & Transformers & \cmark & \goalbox{C} \goalbox{E} \goalbox{IMP} \filledgoalbox{INT} \goalbox{R} \\
\cite{swamy2021interpreting} \href{https://github.com/epfml/interpret-lm-knowledge}{Experiments} & 19 & 2 & 05/22 & BERT-based LM & \xmark & \filledgoalbox{C} \goalbox{E} \goalbox{IMP} \goalbox{INT} \goalbox{R} \\
\cite{wu2021polyjuice} \href{https://github.com/tongshuangwu/polyjuice}{Polyjuice} & 90 & 16 & 08/22 & - & \cmark & \goalbox{C} \filledgoalbox{E} \goalbox{IMP} \goalbox{INT} \goalbox{R}\\
\cite{wang2022interpretability} \href{https://github.com/redwoodresearch/Easy-Transformer}{TransformerLens} & 48 & 161 & 01/23 & GPT2-small & \xmark & \goalbox{C} \filledgoalbox{E} \goalbox{IMP} \goalbox{INT} \goalbox{R}\\
\cite{menon2022visual} - & - & - & - & Vision-LM & \cmark & \goalbox{C} \goalbox{E} \filledgoalbox{IMP} \filledgoalbox{INT} \goalbox{R}\\
\cite{gao2023chatgpt} \href{https://github.com/ArrogantL/ChatGPT4CausalReasoning}{Experiments} & 17 & 0 & 10/23 & ChatGPT & \xmark & \goalbox{C} \goalbox{E} \goalbox{IMP} \goalbox{INT} \filledgoalbox{R} \\
\cite{pan2023unifying} - & - & - & - & LLMs & \cmark & \goalbox{C} \goalbox{E} \goalbox{IMP} \filledgoalbox{INT} \goalbox{R}\\
\cite{conmy2023towards} \href{https://github.com/ArthurConmy/Automatic-Circuit-Discovery}{ACDC} & 105 & 23 & 11/23 & Transformers & \cmark & \goalbox{C} \goalbox{E} \goalbox{IMP} \filledgoalbox{INT} \goalbox{R} \\
\cite{he2022rethinking} \href{https://github.com/HornHehhf/RR}{RR} & 38 & 2 & 02/23 & LLMs & \cmark & \goalbox{C} \filledgoalbox{E} \filledgoalbox{IMP} \goalbox{INT} \goalbox{R} \\
\cite{yoran2023answering} \href{https://github.com/oriyor/reasoning-on-cots}{MCR} & 71 & 9 & 01/24 & LLMs & \cmark & \goalbox{C} \goalbox{E} \goalbox{IMP} \goalbox{INT} \filledgoalbox{R} \\
\cite{sarti2023inseq} \href{https://github.com/inseq-team/inseq}{Inseq} & 250 & 26 & 01/24 & SeqGen models & \cmark & \goalbox{C} \goalbox{E} \goalbox{IMP} \filledgoalbox{INT} \goalbox{R} \\
\cite{wu2023interpretability} \href{https://github.com/frankaging/align-transformers}{Boundless DAS} & 0 & 17 & 01/24 & LLMs & \cmark & \goalbox{C} \filledgoalbox{E} \goalbox{IMP} \goalbox{INT} \goalbox{R} \\
\cite{li2023towards} \href{https://github.com/paihengxu/XICL}{XICL} & 1 & 3 & 11/23 & LLMs & \cmark & \goalbox{C} \filledgoalbox{E} \goalbox{IMP} \goalbox{INT} \goalbox{R} \\
\cite{chen2023lmexplainer} LMExplainer & - & - & - & LLMs & \cmark & \goalbox{C} \filledgoalbox{E} \goalbox{IMP} \goalbox{INT} \goalbox{R} \\
\cite{gao2023chat} Chat-REC & - & - & - & Rec. systems & \xmark & \goalbox{C} \filledgoalbox{E} \filledgoalbox{IMP} \goalbox{INT} \goalbox{R} \\
\midrule
\cite{zhang2022improved} \href{https://github.com/moqingyan/dsr-lm}{DSRLM} & 9 & 1 & 07/23 & LLMs & \cmark & \goalbox{C} \goalbox{E} \goalbox{IMP} \goalbox{INT} \filledgoalbox{R} \\
\cite{singh2023explaining} \href{https://github.com/csinva/imodelsX}{SASC} & 61 & 14 & 01/24 & LLMs & \cmark & \goalbox{C} \filledgoalbox{E} \goalbox{IMP} \goalbox{INT} \goalbox{R} \\
\cite{li2022explanations} - & - & - & - & LLMs & \cmark & \goalbox{C} \filledgoalbox{E} \filledgoalbox{IMP} \goalbox{INT} \goalbox{R} \\
\cite{ye2022unreliability} \href{https://github.com/xiye17/TextualExplInContext}{TextualExplInContext} & 11 & 2 & 02/23 & LLMs & \cmark & \goalbox{C} \filledgoalbox{E} \filledgoalbox{IMP} \goalbox{INT} \goalbox{R}\\
\cite{turpin2023language} \href{https://github.com/milesaturpin/cot-unfaithfulness}{Experiments} & 25 & 9 & 03/23 & LLMs & \cmark & \goalbox{C} \filledgoalbox{E} \goalbox{IMP} \goalbox{INT} \goalbox{R}\\
\cite{kang2023explainable} AutoSD & - & - & - & Debugging models & \xmark & \goalbox{C} \filledgoalbox{E} \filledgoalbox{IMP} \goalbox{INT} \goalbox{R} \\
\cite{krishna2023post} AMPLIFY & - & - & - & LLMs & \cmark & \goalbox{C} \goalbox{E} \filledgoalbox{IMP} \goalbox{INT} \goalbox{R} \\
\cite{yang2023language} \href{https://github.com/YueYANG1996/LaBo}{Labo} & 51 & 4 & 12/23 & CBM & \xmark & \goalbox{C} \goalbox{E} \filledgoalbox{IMP} \goalbox{INT} \goalbox{R} \\
\cite{bitton2023breaking} \href{https://whoops-benchmark.github.io/}{WHOOPS!} & - & - & - & LLMs & \cmark & \goalbox{C} \filledgoalbox{E} \goalbox{IMP} \goalbox{INT} \goalbox{R} \\
\cite{shi2023chatgraph} \href{https://github.com/sycny/ChatGraph}{Chatgraph} & 2 & 0 & 07/23 & LLMs & \cmark & \goalbox{C} \goalbox{E} \goalbox{IMP} \filledgoalbox{INT} \goalbox{R} \\
\bottomrule
\end{tabular}} 
\caption{Synthesis of recent application papers, summarising engagement indicators as of January 2024, update timelines, model specificity, and the overarching aims of each study. In the first section of the table, \textit{To Explain} papers are listed, and \textit{As Feature} works in the second. Stars, forks, and last updates are not reported (-) for papers lacking associated repositories. Target is the specific focus of the study, such as a particular type of language model. Agnostic indicates whether the study is model-agnostic or not. The goal represents the primary objective of each study: comparison of models (C), explanation (E), improvement (IMP), interpretability (INT), and reasoning (R).}


\label{tab:studies}
\end{table*}

